FaceShop: Deep Sketch-based Face Image Editing

We present a novel system for sketch-based face image editing, enabling users to edit images intuitively by sketching a few strokes on a region of interest. Our interface features tools to express a desired image manipulation by providing both geometry and color constraints as user-drawn strokes. As an alternative to the direct user input, our proposed system naturally supports a copy-paste mode, which allows users to edit a given image region by using parts of another exemplar image without the need of hand-drawn sketching at all. The proposed interface runs in real-time and facilitates an interactive and iterative workflow to quickly express the intended edits. Our system is based on a novel sketch domain and a convolutional neural network trained end-to-end to automatically learn to render image regions corresponding to the input strokes. To achieve high quality and semantically consistent results we train our neural network on two simultaneous tasks, namely image completion and image translation. To the best of our knowledge, we are the first to combine these two tasks in a unified framework for interactive image editing. Our results show that the proposed sketch domain, network architecture, and training procedure generalize well to real user input and enable high quality synthesis results without additional post-processing.

==> results.tex <==
\section{Results}
\label{sec:results}

We next present ablation studies to demonstrate the benefits of various components of our system (Section~\ref{subsec:ablation}), followed by image editing results and comparisons to related techniques (Sections~\ref{sec:sketch-based-face-image-editing}, \ref{sec:smart-copy-paste}).

\subsection{Ablation Studies}
\label{subsec:ablation}

We first demonstrate the effect of our automatically constructed sketch domain (Section~\ref{sec:sketch-domain}). The key observation is that, while both raw HED edge maps~\cite{Xie_2015_ICCV} and our sketch domain lead to very similar conditional image completion, our sketch domain generalizes better to free hand sketches provided by users. Figure~\ref{fig:training_like_hed_vs_hedprep} compares conditional image completion based on automatically constructed (using the input image itself) HED edge maps and our sketch domain, showing that both lead to high quality results. In contrast, Figure~\ref{fig:hed_vs_hedprep} illustrates results from free hand user sketches. Synthesized results  with HED (middle column) are blurrier and show some artifacts. Because the system is trained on highly accurate HED edge maps, artifacts in the user input translates into artifacts in the output. Our sketch domain leaves some ambiguity between image structures and sketch strokes, which enables the system to avoid artifacts when the user input is inaccurate.

%* general results on training-like test input
%* results edge maps vs sketch domain

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{images/training_like.pdf}
\caption{Editing results on training-like data for HED edges and our proposed sketch domain. Both lead to high quality conditional image completion.}
\label{fig:training_like_hed_vs_hedprep}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{images/user_input.pdf}
\caption{Editing results on real user input for a system trained using HED edges (middle) and our proposed sketch domain (right). Using HED edges, the system translates artifacts in the user input into artifacts in the output. Our sketch domain leaves some ambiguity between image structures and sketch edges, allowing the system to suppress inaccuracies in the user input.}
\label{fig:hed_vs_hedprep}
\end{figure}

Figure~\ref{fig:rot_vs_norot} illustrates the benefit of using randomly rotated masks during training. Training only with axis aligned masks suffers from overfitting, and artifacts occur with non-axis aligned and arbitrarily shaped masks, as typically provided by users. On the other hand, our approach avoids these issues.

%* mask vs no mask, axis-aligned vs rotated masks

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{images/rot_vs_norot.pdf}
\caption{Comparison of training with axis-aligned masks (middle) and randomly rotated masks (right). Randomly rotating masks avoids overfitting and generalizes to arbitrarily shaped masks.}
\label{fig:rot_vs_norot}
\end{figure}

We demonstrate the need of including the mask in the input to the discriminators (see Figure~\ref{fig:dis_arch}) in Figure~\ref{fig:dismask_vs_nodismask}. Without providing the mask to the discriminator subtle artifacts around the mask boundaries occur, while our approach eliminates them.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{images/dismask_vs_nodismask.pdf}
\caption{Subtle artifacts appear if the mask is not provided as an input to the discriminators (middle). Our approach includes the mask in the discriminator input and avoids these issues (right).}
\label{fig:dismask_vs_nodismask}
\end{figure}

Finally, Figure~\ref{fig:noise} highlights the importance of using skip connections in the conditional generator (Figure~\ref{fig:gen_arch}) and a noise layer in its input. Without these provisions, the conditional completion network produces unrealistic textures (second image from the left). In contrast, with our approach we obtain a high quality output (third and fourth image). We show two results with different noise patterns to emphasize the influence of the noise on the texture details, visualized by the difference image on the right. 
%* noise, skips

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{images/noise.pdf}
\caption{Including a noise layer is important to produce realistic textures. Without it, synthesized textures exhibit artifacts (second image from left). We show results with two noise patterns (third and fourth image), and highlight the influence of the noise on texture details using a difference image (right).}
\label{fig:noise}
\end{figure}

\subsection{Sketch-based Face Image Editing}
\label{sec:sketch-based-face-image-editing}

\begin{figure*}[t]
\centering
\includegraphics[width=0.96\textwidth]{images/sketch_results1_v2.pdf}
\caption{Results using sketching with our system. The examples shown here include editing of nose shape, facial expression (open or close mouth), hairstyle, eyes (open or close eyes, gaze direction, glasses), and face shape. Synthesized face regions exhibit plausible shading and texture detail.}
\label{fig:sketch_results}
\end{figure*}

Figure~\ref{fig:sketch_results} shows various results obtained with our system using sketching. They include editing operations to change the nose shape, facial expression (open or close mouth), hairstyle, eyes (open or close eyes, gaze direction, glasses), and face shape. These examples demonstrate that by providing simple sketches, users can obtain predictive, high quality results with our system. Edges in the user sketches intuitively determine the output, while the system is robust to small imperfections in the sketches, largely avoiding any visible artifacts in the output. Synthesized face regions exhibit plausible shading and texture detail. In addition, these results underline the flexibility of our system, which is able to realize a variety of intended user edits without being restricted to specific operations (like opening eyes~\cite{dolhansky2017eye}).

%* general sketch results with some blabla
%* same input image with different variations of similar edits (e.g. different noses, mouths) to show that it does not just randomly replace the part but that it is sensitive to different sketches
%* input image and then pairs of results (mask/sketch with bare visible image as background, result)
%* examples
%- noses
%- mouths
%- mustache, hair (add and remove)
%- remove glasses, add glasses
%- close eyes, add wrinkles, remove wrinkles, change gaze
%- change head shape

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{images/coloring_results.pdf}
\caption{Results using sketching and coloring. The unmodified input images are shown in Figure~\ref{fig:sketch_results} in rows three and six, leftmost column.}
\label{fig:coloring_results}
\end{figure*}

Figure~\ref{fig:coloring_results} highlights the color editing functionality of our system, where we show examples of changing eye, makeup, and lip color. This shows that the system is robust to imperfect user input consisting of only rough color strokes, largely avoiding artifacts. 

%* sketch + color results with some blabla

\subsection{Smart Copy-Paste}
\label{sec:smart-copy-paste}

Figure~\ref{fig:cp_vs_poisson} shows results of our smart copy-paste functionality, where we copy the masked sketch domain of a source image into a target image. This allows users to edit images in an example-based manner, without the need to draw free hand sketches. In addition, we compare our results to Poisson image editing~\cite{Perez2003}. The comparison reveals that Poisson image editing often produces artifacts due to mismatches in shading (second, fourth, sixth column) or face geometry (third column) between the source and target images. Our approach is more robust and avoids artifacts, although significant misalignment between source and target still leads to unnatural outputs (third column).

%* copy paste results compared to poisson with blabla

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{images/cp_vs_poisson_v2.pdf}
\caption{Our system supports example-based editing via copy-and-paste. We show input images (first row), copy-paste input (second row), and results from Poisson image editing (third row) and our approach (last row). Note that Poisson image editing copies gradients, while we copy the sketch domain of the source region. While our results are mostly free of artifacts, Poisson image editing often suffers from inconsistencies between source and target images.}
\label{fig:cp_vs_poisson}
\end{figure*}

% * copy paste results compared with eye inpainting with blabla

Our copy-paste approach is generic and can be applied to any image region, subsuming specialized approaches, like the ``open eyes'' functionality in Adobe Photoshop Elements, or the eye inpainting technique by Dohansky et al.~\shortcite{dolhansky2017eye}. We compare our approach to these techniques in Figure~\ref{fig:cp_vs_eye-inpainting}. While Adobe's technique may lead to color artifacts, and Dohansky et al.~\shortcite{dolhansky2017eye} is limited to lower resolution images, our approach leads to crisp, high quality results. 

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{images/cp_vs_eye-inpainting_v2.pdf}
\caption{Our generic copy-paste approach can be used for operations such as opening eyes. We compare to two specialized techniques, Adobe's ``open eyes'' functionality and eye inpainting~\cite{dolhansky2017eye}. Our approach produces high quality results, avoiding color artifacts and providing crisper results compared to Dohansky and Ferrer~\shortcite{dolhansky2017eye}.}
\label{fig:cp_vs_eye-inpainting}
\end{figure*}


